Remote sensing and GPS mobility reveal heat's impact on human activity across diverse climates

Extreme heat is a growing threat to both individual livelihoods and broader economies, killing a growing number of people each year as temperatures rise in many parts of the world and limiting productivity. Many studies document the link between heat waves and mortality or morbidity, and others explore the economic consequences of them, but few are able to determine how populations respond to the shock of extreme heat in day-to-day activity. Toward this end, we investigate the link between human mobility and ambient temperature. Examining Indonesia, India and Mexico, we show that extreme heat reduces mobility by up to 10% in urban settings, with losses concentrated midday. We examine the shape of the relationship, finding that while heat reduces activity, very hot days and very long heat waves may induce more of it, indicating different adaptation. Effects are stronger in poorer areas. Twinning these models with climate projections, we show that without adaptation mobility may fall 1-2% per year on aggregate, with certain seasons and places seeing activity fall by as much as 10%. According to our estimates, small cities will face the highest relative losses and large cities will experience the greatest absolute impacts.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
